Hierarchical complexity of 2-clique-colouring weakly chordal graphs and perfect graphs having cliques of size at least 3

A clique of a graph is a maximal set of vertices of size at least 2 that induces a complete graph. A $k$-clique-colouring of a graph is a colouring of the vertices with at most $k$ colours such that no clique is monochromatic. D\'efossez proved that the 2-clique-colouring of perfect graphs is a $\Sigma_2^P$-complete problem [J. Graph Theory 62 (2009) 139--156]. We strengthen this result by showing that it is still $\Sigma_2^P$-complete for weakly chordal graphs. We then determine a hierarchy of nested subclasses of weakly chordal graphs whereby each graph class is in a distinct complexity class, namely $\Sigma_2^P$-complete, $\mathcal{NP}$-complete, and $\mathcal{P}$. We solve an open problem posed by Kratochv\'il and Tuza to determine the complexity of 2-clique-colouring of perfect graphs with all cliques having size at least 3 [J. Algorithms 45 (2002), 40--54], proving that it is a $\Sigma_2^P$-complete problem. We then determine a hierarchy of nested subclasses of perfect graphs with all cliques having size at least 3 whereby each graph class is in a distinct complexity class, namely $\Sigma_2^P$-complete, $\mathcal{NP}$-complete, and $\mathcal{P}$.

==> alg/A_i.tex <==
	\begin{algorithm}[h!]
	\label{alg:A_i}
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	\Input{
			$G = (A, B)$, ($k, 1$)-polar graph \\
			$\pi$, a 2-colouring of $G$ \\
			$A_i$, a maximal complete set in partition $A$
	}
	\Output{$yes$, if every clique of $G$ containing a subset of a maximal complete
	set of $A_i$ is polychromatic}
	\caption{$O(n)$-time algorithm to output $yes$, if every
clique of a ($k, 1$)-polar graph containing a subset of maximal complete set
in partition $A$ is polychromatic, for a fixed $k \geq 1$.}
	\BlankLine
	\Begin
	{	
		\eIf{$|\pi(A_i)| \geq 2$}
		{
			\For{
				$i=1$ \emph{\KwTo} $|A_i|$
			}
			{
        		$answer \longleftarrow recursive(A_i \setminus \{x_i\})$\;
    	    	\If{$answer = no$}
    	    	{
					\Return{$no$\;}
    	    	}
	        }
			\Return{$yes$\;}
		}
		{
			$B_i \longleftarrow \displaystyle\bigcap_{v \in A_{i}} (N(v) \cap B)$\;
			\eIf{$|\pi(A_i \cup B_i)| \geq 2$}
			{
				\Return{$yes$\;}
	        }
	        {
				\Return{$no$\;}	        	
	        }
		}
	}
	\end{algorithm}


==> alg/reduction-np-2.tex <==
	\begin{algorithm}[h!]
	\label{alg:reducion-np-2}
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	\Input{
			$G = (A, B)$, a ($3, 1$)-polar graph
	}
	\Output{$G^\prime$, a ($2, 1$)-polar graph.}
	\caption{An $O(n^2)$-time algorithm to output a ($2, 1$)-polar graph given a
	($3, 1$)-polar graph as input, where every triangle $K$ of the given ($3,
	1$)-polar graph is replaced by an edge $K^\prime$, such that $K$ and $K^\prime$
	are either in the same case $K4$ with $\displaystyle \bigcup_{v \in K}
	N_B(v) = \displaystyle \bigcup_{v \in K^\prime} N_B(v)$ or $\max\{|N_B(v)|, v
	\in K\} = \max\{|N_B(u)|, u \in K^\prime\}$.}
	\BlankLine
	\Begin
	{	
		\ForEach
		{
			maximal complete set $K = \{v_1, v_2, v_3\} \subseteq A$
		}
		{
			$V^\prime \longleftarrow \{u_1, u_2\}$\;
			$E^\prime \longleftarrow \{(u_1, u_2)\}$\;
			\eIf{$\nexists u \in K, N_B(u) = \emptyset \wedge \nexists v, w \in K, v
			\neq w, N_B(v) \subseteq N_B(w) \wedge \displaystyle \bigcap_{z \in K} N_B(z) =
			\emptyset$}
			{
					$E^\prime \longleftarrow E^\prime \cup \{(u_1, x) \mid x \in N_B(v_1)\}$\; 
					$E^\prime \longleftarrow E^\prime \cup \{(u_2, x) \mid x \in ((N_B(v_2)
					\cup N_B(v_3)) \setminus N_B(v_1))\}$\; 
			}
			{
				$N_B^{max} \longleftarrow N_B(\ell)$, s.t. $\ell \in K, |N_B(\ell)| =
				\max \{|N_B(v_1)|, |N_B(v_2)|, |N_B(v_3)|\}$\; 
				$E^\prime \longleftarrow E^\prime \cup \{(u_1,
				x) \mid x \in N_B^{max}\}$\; }
			
			$G \longleftarrow G[V(G) \setminus K]$\;
			$V(G) \longleftarrow V(G) \cup V^\prime$\;
			$E(G) \longleftarrow E(G) \cup E^\prime$\; 
			
	    }
	    \Return{$G$\;}
	}
	\end{algorithm}


==> alg/test2-clique-colouring.tex <==
	\begin{algorithm}[h!]
	\label{alg:test2-clique-colouring}
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	\Input{
			$G = (A, B)$, ($k, 1$)-polar graph \\
			$\pi$, a 2-colouring of $G$ \\
	}
	\Output{$yes$, if $\pi$ is a 2-clique-colouring o $G$.}
	\caption{$O(n^2)$-time algorithm to output $yes$, if $\pi$ is a
	clique-colouring of a ($k, 1$)-polar graph, for a fixed $k \geq 1$.}
	\BlankLine
	\Begin
	{	
		\ForEach
		{
			maximal complete set $A^\prime \in A$
		}
		{
        	$answer \longleftarrow Algorithm~\ref{alg:A_i}(G, \pi, A^\prime)$\;
    	   	\If{$answer = no$}
    	   	{
				\Return{$no$\;}
    	   	}
		}
		\ForEach
		{
			maximal complete set $A^\prime \in A$
		}
		{
			\ForEach
			{
				$v \in A^\prime$
			}
			{
	    	   	\If{$N_B(v) = B$}
	    	   	{
					\Return{$yes$\;}
	    	  	}
    	  	}
	    }
		\eIf{$|\pi(B)| \geq 2$}
		{
			\Return{$yes$\;}
	    }
	    {
			\Return{$no$\;}	        	
		}
	}
	\end{algorithm}


==> lem/31polargraphs.tex <==
\begin{proof}

First, we prove the former assertion. For the sake of
contradiction, suppose $\displaystyle \bigcup_{z \in K} N_B(z)$ is
monochromatic for some 2-clique-colouring of $G$. Without loss of generality,
suppose that all vertices in $\displaystyle \bigcup_{z \in K} N_B(z)$ have colour 1. 
Hence, every vertex $z \in K$ has to receive
colour 2, otherwise $\{z\} \cup N_B(z)$ is a monochromatic clique. On the other
hand, if every vertex $z \in K$ has the same colour, then $K$ is a monochromatic
clique, a contradiction. Hence, we conclude the proof of the former assertion.

Now, we prove the latter assertion. Suppose $K$ is an edge. We have four cases.

\begin{enumerate}
  \item $K$ is in case $\ka$. Let $u \in K, N_B(u) = \emptyset$. Let $v \in K
  \setminus \{u\}$.
  If $N_B(v) = \emptyset$, then give colour 1 to $v$ and colour 2 to $u$.  
  Otherwise, i.e. $N_B(v) \neq \emptyset$, give colour 1 to $v$ if there
  exists a vertex in $N_B(v)$ with colour 2, or else we assign colour 2 to $v$.
  Moreover, give colour 1 to $u$, if vertex $v$ has colour 2, or else we assign
  colour 1 to $u$.
  \item $K$ is in case $\kb$. Let $v, w \in K, v \neq w, N_B(v) \subseteq
  N_B(w)$. Assign colour 1 to $v$ if there exists a vertex in $N_B(v)$ with colour 1, or else assign
  colour 2 to $v$. Assign colour 2 to $w$ if vertex $v$ received colour 1, or
  else assign colour 1 to $w$.
  \item $K$ is in case $\kc$. Assign colour 1 to every vertex in $K$, if there
  exists a vertex in $\displaystyle \bigcap_{z \in K} N_B(z)$ with colour 2, or else
  assign colour 2 to every vertex in $K$.
  \item $K$ is in case $\kd$. Let $u, v \in K$, $u \neq v$. By hyphotesis,
  $N_B(u) \cup N_B(v)$ is polychromatic. Hence, $N_B(u)$ or $N_B(v)$ is polychromatic. Without loss of
  generality, suppose $N_B(u)$ is polychromatic. Assign colour 1 to $v$ if there
  exists a vertex in $N_B(v)$ with colour 2, or else assign colour 2 to $v$.
  Assign colour 1 to $u$, if vertex $v$ received colour 1, or else assign colour
  2 to $u$.
\end{enumerate}
   
Now, suppose $K$ is a triangle. We have four cases.

\begin{enumerate}
  \item $K$ is in case $\ka$. Let $u \in K, N_B(u) = \emptyset$. Let $v, w \in K \setminus \{u\}$, $v
  \neq w$. If $N_B(v) \cup N_B(w) = \emptyset$, then assign colours 1, 1, and 2
  to $u$, $v$, and $w$ respectively. Now, if $N_B(v) \cup N_B(w)$ is
  monochomatic, then assign colour 1 to $v$ and $w$ if the colour assigned to
  every vertex in $N_B(v) \cup N_B(w)$ is 2, or else we assign colour 1 to $v$
  and $w$. Moreover, assign colour 1 to $u$ if $v$ and $w$ have colour 2, or
  else we assign colour 2 to $u$. Now, if $N_B(v) \cup N_B(w)$ is polychromatic,
  we have two cases. If $N_B(v) \cap N_B(w) \neq \emptyset$, then assign colour
  1 to $v$ and $w$ if there exists a vertex in $N_B(v) \cap N_B(w)$ with colour
  2, or else we assign colour 1 to $v$ and $w$. Moreover, assign colour 1 to $u$
  if $v$ and $w$ have colour 2, or else we assign colour 2 to $u$. If $N_B(v)
  \cap N_B(w) = \emptyset$, assign colour 1 to $v$ (resp. $w$) if there exists a
  vertex in $N_B(v)$ (resp. $N_B(w)$) with colour 2, or else assign colour 2 to
  $v$ (resp. $w$). Moreover, assign colour 1 to $u$ if $v$ or $w$ have colour
  2, or else we assign colour 2 to $u$.
  \item $K$ is in case $\kb$. Let $v, w \in K, v \neq w, N_B(v) \subseteq
  N_B(w)$. Assign colour 1 to $v$ if there exists a vertex in $N_B(v)$ with colour 1, or else assign
  colour 2 to $v$. Assign colour 2 to $w$ if vertex $v$ received colour 1, or
  else assign colour 1 to $w$. Let $u \in K \setminus \{v, w\}$. By hyphotesis,
  $N_B(u) \neq \emptyset$. Assign colour 1 to $u$ if there exists a vertex in
  $N_B(u)$ with colour 2, or else assign colour 2 to $u$.
  \item $K$ is in case $\kc$. Assign colour 1 to every vertex in $K$, if there
  exists a vertex in $\displaystyle \bigcap_{z \in K} N_B(z)$ with colour 2, or else
  assign colour 2 to every vertex in $K$.
  \item $K$ is in case $\kd$. There exists $u, v \in K$, such that $N_B(u) \cup
  N_B(v)$ is polychromatic. Otherwise, $\displaystyle_{z \in K} N_B(z)$ is monochromatic.
  Let $w \in K \setminus \{u, v\}$. We have two cases. Suppose that sets
  $N_B(u)$ and $N_B(v)$ are monochromatic. Assign colour 1 to $u$ (resp.
  colour 2 to $v$) if every vertex in $N_B(u)$ has colour 2 (resp. every vertex
  in $N_B(v)$ has colour 1), or else we assign colour 2 to $v$ (resp. 1 to $w$).
  Moreover, assign colour 1 to $w$ if there exists a vertex in $N_B(w)$ with
  colour 2, or else we assign colour 2 to $w$. Now, suppose that either $N_B(u)$
  or $N_B(v)$ is monochromatic. Without loss of generality, suppose $N_B(u)$ is
  polychromatic. Without loss of generality, suppose $N_B(u)$ is polychromatic. 
  Assign colour 1 to $v$ if there exists a vertex in $N_B(v)$ with colour 2, or
  else assign colour 2 to $v$. Assign colour 1 to $u$, if vertex $v$ received
  colour 1, or else assign colour 2 to $u$. Moreover, assign colour 1 to $w$ if
  there exists a vertex in $N_B(w)$ with colour 2, or else we assign colour 2 to
  $w$.
\end{enumerate}


\end{proof}


==> lem/auxiliarygraphs.tex <==
\begin{proof}
Follows from the fact that in $A(x, y)$ there exists a cycle $x v_1 v_2 \ldots v_{a-2} y$ such that no edge lies in a triangle of $G$.
\end{proof}


==> lem/nptocheck.tex <==
\begin{proof}
Let $\pi$ be a 2-colouring of $G$ and notice that partition $B$ is
also a clique. We prove the correctness of Algorithm~\ref{alg:A_i} by induction.  
Consider a maximal complete set of size $k$ and contained in partition $A$, say
$A_1$. If $A_1$ is monochromatic, then we need to check if $A_1$ is properly
contained in a clique of graph $G$. Let $B_1 = \displaystyle\bigcap_{v \in A_1}
(N(v) \cap B)$. One can check that $A_1 \cup B_1$ is a clique of graph $G$. If
$A_1 \cup B_1$ is monochromatic, then $\pi$ is not a 2-clique-colouring of $G$.
Otherwise, i.e. $A_1 \cup B_1$ is polychromatic, then every clique containing a
vertex $u$ in $A_1$ is polychromatic, since $\{u\} \cup B_1$ is polychromatic.
Now, if $A_1$ is polychromatic, then we need to check whether every clique of
$G$ containing a proper subset of $A_1$ is polychromatic.  

Let $A_{k+1} = A_1 \setminus \{x_1, \ldots, x_{k}\}$, for some $\{x_1, \ldots,
x_{k}\} \subsetneq A_1$. Suppose (as induction hyphotesis) that every clique of
$G$ containing $A_{i}$, for every $1 \leq i \leq k$, is polychromatic.

For the induction step, consider a clique of graph $G$ containing $A_{k+1}$, say
$K$. Then, either $A_{k+1} \subsetneq (K \cap A_1)$ or $A_{k+1} = (K \cap A_1)$.
If $A_{k+1} \subsetneq (K \cap A_1)$, then $K$ contains $A_{j}$, for some $1
\leq j \leq k$, and every clique containing $A_{j}$ is polychromatic.
Otherwise, i.e. $A_{k+1} = (K \cap A_1)$, one can
check that $K = A_{k+1} \cup B_{k+1}$, where $B_{k+1} = \displaystyle\bigcap_{v
\in A_{k+1}} (N(v) \cap B)$.
Suppose $A_{k+1}$ is monochromatic. If $K$ is monochromatic, then $\pi$ is not a
2-clique-colouring of $G$. Otherwise, i.e. $K$ is polychromatic, then every
clique containing a vertex $u$ in $A_{k+1}$ is polychromatic, since $\{u\} \cup
B_{k+1}$ is polychromatic. Now, if $A_{k+1}$ is polychromatic, then we need to
check whether every clique of $G$ containing a proper subset of $A_{k+1}$ is
polychromatic. Notice that $A_{k+1}$ is monochromatic, when $|A_{k+1}| = 1$,
and it is handled properly in the opposite case (i.e., when $A_{k+1}$ is
monochromatic) and the proof of the correctness of Algorithm~\ref{alg:A_i} is
done.

Now, we give the time-complexity of Algorithm~\ref{alg:A_i}. First, there are at
most $|A_i|!$ recursive calls. Second, in one iteration of the algorithm, the
number of steps is upper bounded by the complexity of calculating $B_i$. 
One can design an $O(|B| \log |A_i|)$-time algorithm to calculate $B_i$. Then,
the algorithm is executed in at most $k! \log k |B| = O(n)$ steps.
\end{proof}


==> lem/question.tex <==
\begin{proof}
Follows from the first assertion of Lemma~\ref{lem:31polargraphs}.
\end{proof}

==> thm/2cc21polar.tex <==
\begin{proof}
The problem of 2-clique-colouring a ($2, 1$)-polar graph is in $\mathcal{NP}$:
Theorem~\ref{thm:nptocheck} confirms that to check whether a colouring of a
($2, 1$)-polar graph is a 2-clique-colouring is in $\mathcal{P}$. The problem of
2-clique-colouring a ($2, 1$)-polar graph is $\mathcal{NP}$-hard:
Theorem~\ref{thm:2cc21polarnphar} confirms that for every ($3, 1$)-polar graph
$G$, a ($2, 1$)-polar graph $G^\prime$ is constructed such that $G$ is
2-clique-colourable if, and only if, graph $G^\prime$ is 2-clique-colourable.
Moreover, such construction is done in polynomial-time.
\end{proof}


==> thm/2cc21polarreduction.tex <==
\begin{proof}
We use induction on the number of triangles in partition $A$
of $G$ to prove that $G$ is 2-clique-colourable if and only if $G^\prime$ is
2-clique-colourable. For the sake of conciseness, we prove only one way of the
basis induction. The converse and the step induction follows analogously.

Suppose that there exists only one triangle $K = \{v_1, v_2, v_3\}$ in partition
$A$ of $G$. Let $K^\prime = \{u_1, u_2\}$ be the edge that replaced $K$ in
partition $A$ to obtain graph $G^\prime$. Suppose that there exists a
2-clique-colouring of $G$, say $\pi$. Since $\pi$ is a 2-clique-colouring of
$G$, every clique of $G$ containing a subset of a maximal complete set of
partition $A$, other than $K$, is polychromatic.
Let $\pi^\prime$ be a 2-colouring of $G^\prime$, such that $\pi^\prime(v) =
\pi(v)$, for each $v \in V(G) \cap V(G^\prime)$. Hence, every clique of
$G^\prime$ containing a subset of a maximal complete set of partition $A$, other
than $K^\prime$, is polychromatic. Hence, we are left to prove that
every clique containing partition $B$ of $G^\prime$ is polychromatic and every
clique of $G^\prime$ containing a subset of $K^\prime$ is polychromatic. 
If $B$ is a clique of $G$, then $B$ is polychromatic under $\pi$. Clearly, $B$ is also
polychromatic under $\pi^\prime$. Now, suppose $B$ is not a clique of $G$. We
know that every clique of $G$ containing a subset of a maximal complete
set of partition $A$, other than $K$, is polychromatic. In particular,
those cliques also containing $B$. Clearly, those cliques are also polychromatic
in $G^\prime$. Now, if a clique in $G$ contains $B$ and a subset of $K$, then
there is a clique in $G^\prime$ that contains $B$ and at least one vertex of
$K^\prime$, since $\max\{|N_B(v)|, v \in K\} = \max\{|N_B(u)|, u \in K^\prime\}$.
Hence, we are left to prove that every clique of $G^\prime$ containing a subset
of $K^\prime$ is polychromatic. If $K^\prime$ is either in case $\ka$, $\kb$ or
$\kc$, then $\pi^\prime$ can be extended to $G^\prime$, such that every clique
containing a subset of $K^\prime$ is polychromatic
(Lemma~\ref{lem:31polargraphs}). If $K$ is in case $\kd$, then $\displaystyle
\bigcup_{v \in K} N_B(v)$ is polychromatic. Since $\displaystyle
\bigcup_{v \in K} N_B(v) = \displaystyle \bigcup_{v \in K^\prime} N_B(v)$ and 
$\pi^\prime(v) = \pi(v)$, for each $v \in B$, $\displaystyle \bigcup_{v \in
K^\prime} N_B(v)$ is polychromatic. Moreover, also by
Lemma~\ref{lem:31polargraphs}, the colouring $\pi^\prime$ can be extended to
$G^\prime$, such that every clique containing a subset of $K^\prime$ is
polychromatic.
\end{proof}

==> thm/2cc31polar.tex <==
\begin{proof}
The problem of 2-clique-colouring a ($3, 1$)-polar graph is in $\mathcal{NP}$:
Theorem~\ref{thm:nptocheck} confirms that to check whether a colouring of a ($3,
1$)-polar graph is a 2-clique-colouring is in $\mathcal{P}$.


We prove that 2-clique-colouring ($3, 1$)-polar graphs is $\mathcal{NP}$-hard by
reducing {\sc NAE-SAT} to it.
The outline of the proof follows: for every formula $\phi$, a graph $G$
is constructed such that $\phi$ is satisfiable if, and only if, graph $G$ is 2-clique-colourable. 
We finish the proof showing that $G$ is ($3, 1$)-polar.

Let $n$ (resp. $m$) be the number of variables (resp. clauses) in formula $\phi$. 
We define the graph $G$ as follows.

\begin{itemize}
	\item for each variable $x_i$, $1 \leq i \leq n$, we create four vertices
	$x_i$, $x^\prime_i$, $x^{\prime\prime}_i$, and $\overline{x}_i$ with edges $x_i
	x^\prime_i$, $x^\prime_i x^{\prime\prime}_i$, and $x^{\prime\prime}_i
	\overline{x}_i$. Notice that vertices $x_i$ and $\overline{x}_i$ correspond to the
	literals of variable~$x_i$. Moreover, we create edges in order to the set
	$\{x_1, \overline{x}_1, \ldots, x_n, \overline{x}_n\}$ induces a complete subgraph
	of~$G$. 
	\item for each clause $c_j = (l_a, l_b, l_c)$, $1 \leq j \leq m$, we create a
	triangle $c_j$ with three vertices $l_{a_{c_j}}$, $l_{b_{c_j}}$, and
	$l_{c_{c_j}}$. Notice that vertices $l_{a_{c_j}}$, $l_{b_{c_j}}$, and
	$l_{c_{c_j}}$ correspond to the literals of clause $c_j$. Moreover, each
	vertex $l \in \{l_{a_{c_j}}, l_{b_{c_j}}, l_{c_{c_j}}\}$ is adjacent to a
	vertex $\overline{l}$ in $\{x_1, \overline{x}_1, \ldots , x_n,
	\overline{x}_n\}$ if, and only if, the literals correspondent to $l$ and
	$\overline{l}$ are distinct literals of the same variable.
\end{itemize}

Refer to Fig.~\ref{fig:reduction-np} for an example of such construction, given
a formula $\phi = (x_{1} \vee \overline{x_{2}} \vee x_{4}) \wedge ( x_{2} \vee
\overline{x_{3}} \vee \overline{x_{5}} )\wedge ( x_{1} \vee x_{3} \vee x_{5})$.

\begin{figure}[h]
\center
	\includegraphics[scale=0.5]{figs/pdf/reduction-np.pdf}
	\caption{Example for $\phi = ( x_{1} \vee \overline{x_{2}} \vee x_{4}) \wedge 
	( x_{2} \vee \overline{x_{3}} \vee \overline{x_{5}} )\wedge ( x_{1} \vee
	x_{3} \vee x_{5})$ }
	\label{fig:reduction-np}
\end{figure}

	We claim that formula $\phi$ is satisfiable if, and only if, there exists a
	2-clique-colouring in~$G$.
	
Assume there exists a valuation $v_\phi$ such that $\phi$ is satisfied. 

We give a colouring to the graph $G$ as follows: 
\begin{itemize}
	\item assign colour 1 to $l \in \{x_1, \overline{x}_1, \ldots, x_n,
	\overline{x}_n\}$ if it corresponds to the literal which receives the $true$
	value in $v_\phi$, or else we assign colour 2 to it.
	\item extend the unique colouring to vertices $x^\prime_i$ and
	$x^{\prime\prime}_i$, for each $1 \leq i \leq n$, i.e. assign
	colour 2 to $x^\prime_i$ and colour 1 to $x^{\prime\prime}_i$ if the
	corresponding literal of $x_i$ is $true$ in $v_\phi$, or else we assign colour 
	2 to $x^\prime_i$ and colour 1 to $x^{\prime\prime}_i$.
	\item extend the unique colouring to vertices $l_{a_{c_j}}$,
	$l_{b_{c_j}}$, and $l_{c_{c_j}}$, for each triangle $c_j = \{l_{a_{c_j}},
	l_{b_{c_j}}, l_{c_{c_j}}\}$, $1 \leq j \leq m$, i.e. assign colour 1 to $l \in
	\{l_{a_{c_j}}, l_{b_{c_j}}, l_{c_{c_j}}\}$ if the corresponding opposite
	literal of the same variable is $false$ in $v_\phi$, or else we assign colour 2 to $l$.
\end{itemize}

It still remains to be proved that this is indeed a 2-clique-colouring.

The cliques of size 2 are $x_i x^\prime_i$, $x^\prime_i x^{\prime\prime}_i$, and
$x^{\prime\prime}_i \overline{x}_i$, for each $1 \leq i \leq n$, and
$l\overline{l}$, where $l \in c_j$ and $\overline{l}$ correspond to distinct
literals of the same variable, for each $1 \leq j \leq m$. The above colouring
gives distinct colours to each vertex of a clique of size 2.

The cliques of size at least 3 are $\{x_1, \overline{x}_1, \ldots, x_n,
\overline{x}_n\}$ and triangle $c_j$, for each $1 \leq j \leq m$. The former is
polychromatic, since two vertices which represent distinct literals of the same
variable receive distinct colours. The latter is also polychromatic, since
$(i)$ every vertex of triangle $c_j$ represents a literal of some variable in
$\phi$, $(ii)$ each clause $c_j$ has at least one literal that receives the
$true$ value and at least one literal that receives the $false$ value (recall
we are reducing from {\sc NAE-SAT} problem), and $(iii)$ a vertex in
triangle $c_j$ receives colour 1 if it corresponds to the literal which the
opposite literal of the same variable receives the $false$ value in $v_\phi$, or
else we assign colour 2 to it.

For the converse, we now assume that $G$ is 2-clique-colourable and we consider
any 2-clique-colouring. Recall the vertices $x_i$ and $\overline{x}_i$
have distinct colours, since $x_i x^\prime_i$, $x^\prime_i x^{\prime\prime}_i$,
and $x^{\prime\prime}_i \overline{x}_i$ are cliques. Hence, we define $v_\phi$
in the following way: the literal $x_i$ is assigned $true$ in $v_\phi$ if the
corresponding vertex has colour 1 in the clique-colouring, or else it is
assigned $false$. Since we are considering a 2-clique-colouring, every triangle
$c_j$, $1 \leq j \leq m$ is polychromatic. As a consequence, there exists at
least one literal with $true$ value in $c_j$ and at least one literal with
$false$ value in every clause $c_j$. This proves that $\phi$ is satisfied for
valuation $v_\phi$.

It now remains to be proved that $G$ is a ($3, 1$)-polar graph.
Let $A = \displaystyle \left(\bigcup_{i = 1}^n \{x^\prime_i,
x^{\prime\prime}_i\}\right) \cup \left(\bigcup_{j = 1}^m \{c_j\}\right)$ and $B
= \{x_1, \overline{x}_1, \ldots, x_n, \overline{x}_n\}$ be the partition of
$V(G)$ into two sets. Each connected component of the subgraph induced by set
$A$ (resp. the complementary subgraph induced by set $B$) is either a
triangle or an edge (resp. a vertex). Hence, $G$ is a ($3, 1$)-polar graph.
\end{proof}


==> thm/nptocheck.tex <==
\begin{proof}
The correctness of Algorithm~\ref{alg:test2-clique-colouring} follows.
A clique of $G$ contains at least one vertex of a maximal complete set of
partition $A$ or it is $B$. The first loop of
Algorithm~\ref{alg:test2-clique-colouring} checks whether all cliques in the
former case are polychromatic. The second loop of
Algorithm~\ref{alg:test2-clique-colouring} checks whether $B$ is a clique. If
$B$ is not a clique, then we already check whether the clique which contains $B$
is polychromatic. If $B$ is a clique, then
Algoritm~\ref{alg:test2-clique-colouring} checks whether $B$ is polychromatic.

Now, we give the time-complexity of Algorithm~\ref{alg:test2-clique-colouring}.
The first loop of Algorithm~\ref{alg:test2-clique-colouring} runs at most $n$
times Algorithm~\ref{alg:A_i}, which runs in $O(n)$-time. 
The second loop of Algorithm~\ref{alg:test2-clique-colouring} runs at most $n$
times a comparison, which runs in $O(n)$-time.
Then, Algorithm~\ref{alg:test2-clique-colouring} is executed in at most $O(n^2)$
steps.
\end{proof}


==> thm/question.tex <==
\begin{proof}
The problem of 2-clique-colouring a ($3, 1$)-polar graph is in $\mathcal{NP}$:
Theorem~\ref{thm:nptocheck} confirms that to check whether a colouring of a ($3,
1$)-polar graph is a 2-clique-colouring is in $\mathcal{P}$.


We prove that 2-clique-colouring ($3, 1$)-polar graphs with cliques having size
at least 3 is $\mathcal{NP}$-hard by reducing {\sc NAE-SAT} to it.
The outline of the proof follows: for every formula $\phi$, a graph $G$ is
constructed such that $\phi$ is satisfiable if, and only if, graph $G$ is
2-clique-colourable. We start the proof constructing $G$ and showing that $G$ is
($3, 1$)-polar with all cliques having size at least 3.

Let $n$ (resp. $m$) be the number of variables (resp. clauses) in formula $\phi$. 
We define the graph $G$ as follows.

\begin{itemize}
	\item create a complete set $B^\prime$ with vertices $x_i$, $x^1_i$,
	$x^2_i$, $x^3_i$, and $\overline{x}_i$ for each variable $x_i$, $1 \leq i \leq
	n$. Notice that vertices $x_i$ and $\overline{x}_i$ correspond to the
	literals of variable~$x_i$.
	\item add copies of the auxiliary graph $H(x^1_i, x^2_i, x^3_i)$,
	$H(x_i, \overline{x}_i, x^1_i)$, $H(x_i, \overline{x}_i, x^2_i)$, and
	$H(x_i, \overline{x}_i, x^3_i)$, for $i = 1, \ldots, |X|$.
	\item for each clause $c_j = (l_a, l_b, l_c)$, $1 \leq j \leq m$, add a copy
	of the auxiliary graph $H(l_a, l_b, l_c)$. Notice that vertices $l_a$, $l_b$,
	and $l_c$ are in $B^\prime$, since they correspond to literals of some
	variables in $X$.
\end{itemize}

%Refer to Fig.~\ref{fig:reduction-np} for an example of such construction, given
%a formula $\phi = (x_{1} \vee \overline{x_{2}} \vee x_{4}) \wedge ( x_{2} \vee
%\overline{x_{3}} \vee \overline{x_{5}} )\wedge ( x_{1} \vee x_{3} \vee x_{5})$.

%\begin{figure}[h]
%\center
%	\includegraphics[scale=0.5]{figs/pdf/reduction-np.pdf}
%	\caption{Example for $\phi = ( x_{1} \vee \overline{x_{2}} \vee x_{4}) \wedge 
%	( x_{2} \vee \overline{x_{3}} \vee \overline{x_{5}} )\wedge ( x_{1} \vee
%	x_{3} \vee x_{5})$ }
%	\label{fig:reduction-np}
%\end{figure}

We claim that $G$ is ($3, 1$)-polar with all cliques having size at least 3. In
fact, complete set $B^\prime$ correspond to partition $B$. Moreover, we add
copies of the auxiliary graph $H(x, y, z)$ with $x, y, z \in B^\prime$, i.e. we
add a triangle to $G$ with neighbors only in $B^\prime$. Hence, $V(G) \setminus
B^prime$ only induces edge-disjoint triangles which correspond to partition $A$.
Now, we are left to prove that all cliques have size at least 3. For each added
copy of the auxiliary graph $H(x, y, z)$ with $x, y, z \in B^\prime$, all edges
lies in a triangle (see Fig.~\ref{fig:question}). Clearly, all edges induced
by the complete set $B^\prime$ lies in a triangle and the claim follows. 

Now, we claim that formula $\phi$ is satisfiable if, and only if, there exists a
2-clique-colouring in~$G$.
	
Assume there exists a valuation $v_\phi$ such that $\phi$ is satisfied. 

We give a colouring to the graph $G$ as follows: 
\begin{itemize}
	\item assign colour 1 to $l \in \{x_1, \overline{x}_1, \ldots, x_n,
	\overline{x}_n\} \subset B^\prime$ if it corresponds to the literal which
	receives the $true$ value in $v_\phi$, or else we assign
	colour 2 to it.
	\item assign colours 1 and 2 to $x^1_i$, $x^2_i$, $x^3_i$, for each $1 \leq i
	\leq n$.
	\item extend the colouring to vertices of each copy of the auxiliary graph
	$H(\cdot, \cdot, \cdot)$ (we shall see that it is doable in what follows).
\end{itemize}

It still remains to be proved that this is indeed a 2-clique-colouring.

The complete set $B$ is polychromatic, since we assign distinct colours to each
$x_i$ and $\overline{x}_i$, for each $1 \leq i \leq n$. Now, we are left to
prove that every clique of $G$ containing a subset of every auxiliary graph
$H(\cdot, \cdot, \cdot) \cap A$ is polychromatic. All added copies of the
auxiliary graph $H(\cdot, \cdot, \cdot)$ are in one of the following cases.
\begin{itemize}
  \item $H(x^1_i, x^2_i, x^3_i)$, for each variable $x_i$, $1 \leq i \leq n$.
  Notice that we assign colours 1 and 2 to $x^1_i$, $x^2_i$, and $x^3_i$.
  \item $H(x_i, \overline{x}_i, x^k_i)$, for each variable $x_i$ and $1 \leq k
  \leq 3$. Notice that we assign distint colours to $x_i, \overline{x}_i$. 
  \item $H(l_a, l_b, l_c)$, for each clause $c_j = (l_a, l_b, l_c)$, $1 \leq j
  \leq m$.
  Notice that we assign colours 1 and 2 to $l_a$, $l_b$, and $l_c$ (recall we are reducing
  from $NAE-SAT$).
\end{itemize}
Hence, follows by the second assertion of Lemma~\ref{lem:31polargraphs} that
every clique of $G$ containing a subset of every auxiliary graph
$H(\cdot, \cdot, \cdot) \cap A$ is polychromatic.

For the converse, we now assume that $G$ is 2-clique-colourable and we consider
any 2-clique-colouring. We claim that $\{x_i, \overline{x}_i\} \subset B$
is polychromatic for each variable $x_i$, for each $1 \leq i \leq n$. For the
sake of contradiction, suppose that $x_i$ and $\overline{x}_i$ have the same
colour. Consider the auxiliary graph $H(x_i, \overline{x}_i, x^k_i) \cap A$,
for each $1 \leq k \leq 3$. Follows from the first assertion of
Lemma~\ref{lem:31polargraphs} that $\{x_i, \overline{x}_i, x^k_i\}$ is
polychromatic, i.e. $x^k_i$ receive a distinct colour. We are considering a
2-clique-colouring of $G$, then $x^1_i$, $x^2_i$, and $x^3_i$ have the same
colour. Now, consider the auxiliary graph $H(x^1_i, x^2_i, x^3_i) \cap A$.
Follows from the counterpositive of the first assertion of
Lemma~\ref{lem:31polargraphs} that $G$ does not have a 2-clique-colouring, a
contradiction with our assumptions. Hence, $x_i$ and $\overline{x}_i$ have
distinct colours, for each $1 \leq i \leq n$. Now, we prove that $\{l_a, l_b,
l_c\} \subset B$ is polychromatic for each clause $c_j = (l_a, l_b, l_c)$, $1
\leq j \leq m$. Consider the auxiliary graph $H(l_a, l_b, l_c) \cap A$.
Follows from the first assertion of Lemma~\ref{lem:31polargraphs} that $\{l_a,
l_b, l_c\}$ is polychromatic. As a consequence, there exists at
least one literal with $true$ value in $c_j$ and at least one literal with
$false$ value in every clause $c$. This proves that $\phi$ is satisfied for
valuation $v_\phi$.
\end{proof}


==> thm/weaklychordal.tex <==
\begin{proof}
Deciding whether a graph has a 2-clique-colouring is in $\Sigma_2^P$: a 2-partition of the graph which is a 2-clique-colouring
is a certificate. Checking whether a 2-partition is a 2-clique-colouring is in $co\mathcal{NP}$: a monochromatic clique is a certificate  
to its complement problem and can be checked in polynomial time if it is indeed monochromatic.

We prove that 2-clique-colouring weakly chordal graphs is $\Sigma_2^P$-Complete
by reducing {\sc QSAT2} to it.
The outline of the proof follows: for every formula $\Psi=(X,Y, D)$, a graph $G$ is 
constructed such that $\Psi$ is satisfiable if, and only if, graph $G$ is
2-clique-colourable.
We finish the proof showing that $G$ is a weakly chordal graph.


We define the graph $G$ as follows:

\begin{itemize}
	\item for each variable $x_i$, we create two vertices $x_i$ and $\overline{x}_i$ ;
	\item for each variable $y_j$, we create three vertices $y_j$, $y^\prime_j$, and $\overline{y}_j$ with edges $y_j y^\prime_j$, and $y^\prime_j \overline{y}_j$; 
	\item we create a vertex $v$ and edges in order to the set
$\{x_1, \overline{x}_1, \ldots , x_n, \overline{x}_n, y_1, \overline{y}_1, \ldots, y_m, \overline{y}_m, v\}$ induces a complete subgraph of $G$ minus the
matching $\{\{x_1, \overline{x}_1\}, \ldots , \{x_n, \overline{x}_n\}, \{y_1, \overline{y}_1\}, \ldots, \{y_m, \overline{y}_m\}\}$.
	\item add copies of the auxiliary graph $NAS(x_i, \overline{x}_i)$, for $i = 1, \ldots, |X|$, 
	\item add copies of the auxiliary graph $AK( \overline{y}_j, y_{j+1})$, for $j = 1, \ldots, |Y|-1$, and 
	\item add a copy of $AK(\overline{y}_m, v)$.
	\item for each implicant $d_k$, we create vertices $d_k, d^\prime_k$, $d^{\prime\prime}_k$, and we add the edges $d_k d^\prime_k$, $d^\prime_k d^{\prime \prime}_k$, $d^{\prime\prime}_k v$, and $d_k v$. Moreover, each vertex $d_k$ is adjacent to a vertex $l$ in $\{x_1, \overline{x}_1, \ldots , x_n, \overline{x}_n, y_1, \overline{y}_1, \ldots, y_m, \overline{y}_m, v\}$ if, and only if, the literal correspondent to $\overline{l}$ is not in the implicant correspondent to vertex $d_k$. 
\end{itemize}

Refer to Fig.~\ref{fig:reduction} for an example of such construction, given a formula $\Psi = (x_1 \vee \overline{x}_2 \vee y_2) \wedge (x_1 \vee x_3 \vee \overline{y}_2) \wedge ( \overline{x}_1 \vee \overline{x}_2 \vee y_1)$.

\begin{figure}[h]
\centering
		\includegraphics[scale=0.5]{figs/pdf/reduction.pdf}
	\caption{Example for $\Psi = (x_1 \vee \overline{x}_2 \vee y_2) \wedge (x_1 \vee x_3 \vee \overline{y}_2) \wedge ( \overline{x}_1 \vee \overline{x}_2 \vee y_1)$, where $NAS$ and $AK$ denotes the respectively auxiliary graphs.}
	\label{fig:reduction}
\end{figure}

We claim that $\Psi$ has a solution if and only if the graph $G$ is 2-clique-colourable.
 
For every $i$, the vertices $x_i$ and $\overline{x}_i$ will have opposite
colours in any 2-clique-colouring of $G$ (Lemma~\ref{lem:auxiliarygraphs}).
The set $\{y_1, y_2, \ldots, y_{|Y|}, \overline{y}_1, \overline{y}_2, \ldots, \overline{y}_m, v\}$ is monochromatic. Indeed, $y_j$, $\overline{y}_j$, $y_{j+1}$ have the same colour, since for $j = 1, \ldots, |Y| - 1$, $y_j y^\prime_j$, $y^\prime_j \overline{y}_j$ are cliques, $\overline{y}_j y_{j+1}$ (resp. $\overline{y}_{|Y|} v$) have the same colour by Lemma~\ref{lem:auxiliarygraphs}.   
Finally, $d_1$, $d_2$, \ldots, $d_{|D|}$ will have the same colour and opposite to the one of $v$.

Assume there exists a valuation $v_X$ such that $\Psi$ is satisfied for any valuation of $Y$.

We give a colouring to the graph $G$ as follows: 
\begin{itemize}
	\item assign colour 1 to $y_j$, $\overline{y}_j$, $j = 1, \ldots, |Y|$, $d^\prime_k$, $k = 1, \ldots, |D|$, and $v$;
	\item assign colour 2 to $y^\prime_j$, for $j = 1, \ldots, |Y|$, and
	\item assign colour 2 to $d_k$, $d^{\prime \prime}_k$, for $k = 1, \ldots, |D|$.
	\item extend the unique colouring to the $|Y|-1$ copies of the auxiliary graph $AK(\overline{y}_j, y_{j+1})$, for $j = 1, \ldots, |Y| - 1$ and $AK(\overline{y}_{|Y|}, v)$.
	\item assign colour 1 to $x_i$ if the corresponding variable is $true$ in
	$v_X$, or else we assign colour 2 to it.
	\item assign colour 2 to $\overline{x}_i$ if the corresponding variable is $true$ in $v_X$, or else we assign colour 1 to it.
	\item extend the unique colouring to the $|X|$ copies os the auxiliary graph $NAS(x_i, \overline{x}_i)$
\end{itemize}

It still remains to be proved that this is indeed a 2-clique-colouring. Let us assume that
it is not the case and that there exists a maximal clique $K$ of $G$ that is monochromatic.
Clearly, $K$ is not contained in a copy of any auxiliary graph, and that it does
not contain any vertex of type $y^\prime_j$, $d^\prime_k$, or $d^{\prime \prime}_k$. 
As $v$ is adjacent to all other vertices
(which are the $x_i$, $\overline{x}_i$, $y_j$, $\overline{y}_j$, and $d_k$), we deduce that $v \in K$ and
subsequently that all vertices of $K$ have colour 1. Moreover, $K$ contains exactly one
vertex among $x_i$ and $\overline{x}_i$, for $i = 1, \ldots, |X|$, i.e. the one corresponding to the literal which is true
in $v_X$, and similarly exactly one vertex among $y_j$ and $\overline{y}_j$, for every $j = 1, \ldots, |Y|$. We remark that
$K$ does not contain any $d_k$ since they have colour 2.
Then we define a valuation $v_Y$ in the following way: if $y_j \in K$, then $v_Y$ assigns
value $true$ to the corresponding variable, or else the value $false$. Thus, the literals
corresponding to the vertices of $K \setminus \{v\}$ are exactly those that are $true$ in the total
valuation $(v_X,v_Y)$. Let us consider now any $d_k$. Since $K$ is maximal, $d_k$ is not adjacent
to at least one vertex of $K$, and by construction of $G$ this means the corresponding
implicant is false.
As a result we have found a valuation $v_Y$ such that all implicants are false, which
contradicts the definition of $v_X$. Hence, there is no monochromatic clique and
we have a 2-clique-colouring.

For the converse, we now assume that $G$ is 2-clique-colourable and we consider any 2-clique-colouring.
Without loss of generality, we can assume that $v$ has colour 1. Then, $y_j$ and $\overline{y}_j$, for $j = 1, \ldots, |Y|$, also
have colour 1, and $d_k$, for $k = 1, \ldots, |D|$, have colour 2.

As for every $i$ the vertices $x_i$ and $\overline{x}_i$ have opposite colours, we define $v_X$ in the
following way: the literal $x_i$ is assigned $true$ in $v_X$ if the corresponding vertex has
colour 1 in the clique-colouring, or else it is assigned $false$.
Let $v_Y$ be any valuation of $Y$. Consider the clique $K$ that contains $v$ and the vertices
corresponding to literals which are $true$ in the total valuation $(v_X, v_Y)$. Since all
those vertices have colour 1, it follows that $K$ cannot be maximal (because we have
a 2-clique-colouring). As a consequence, there exists some $d_k$ which is adjacent to all
vertices of $K$, and thus the corresponding implicant is $true$ in that valuation.
This proves that $\Psi$ is satisfied for any valuation $v_Y$ and consequently that $v_X$ has
the right property.

It now remains to be proved that $G$ is a weakly chordal graph. One can check
that $G$ is $C_{\ell \geq 5}$-free.
Now, we prove that $G$ is $\overline{C}_{\ell \geq 6}$-free.

Let $H$ be an anti-hole of $G$ of size at least 6. 
Clearly, any vertex of $H$ has degree at least 3. Hence, we examine the vertices of $G$ with degree at least 3.
Let $S = \{x_i, \overline{x}_i, y_j, \overline{y}_j, v \mid 1 \leq i \leq |X|, 1 \leq j \leq |Y|\}$.
Let $R = \{d_k | 1 \leq k \leq |D|\}$.
The vertices of degree at least 3 are the vertices of the auxiliary graphs, $S$, and $R$.

Let $A$ a subset of $H$ with 3 vertices. Then,
\begin{itemize}
  \item $A$ is not a subset of $V(NAS(x, y)) \setminus \{x, y\}$. Indeed, one can check that no vertex in $V(NAS(x, y)) \setminus \{x, y\}$ is a vertex in $H$.
  \item $A$ is not a subset of $V(AK(x, y)) \setminus \{x, y\}$. Indeed, one can check that no vertex in $V(NAS(x, y)) \setminus \{x, y\}$ is a vertex in $H$.
  \item $A$ is not a subset of $R$. Indeed, 3 vertices of $R$ induce a $\overline{K_3}$.
  \item $A$ is not a subset of $S$. For the sake of contradiction, suppose $A \subseteq S$. $H \setminus S \subseteq R$, since only vertices in $S$ have degree at least three and may be contained in $H$.  Every vertex of $S \cap H$ has a non-neighbor in $R \cap H$, since a vertex in $S$ has at most one non-neighbor in $S$ and every vertex in $H$ has two non-neighbors.  If $|R \cap H| = 0$, then every vertex in $H$ has at most one non-neighbor (contradiction). If $|R \cap H| > 1$, then one can check that only two vertices in $S \cap H$ may have two non-neighbors (contradiction, $H$ has size at least 5).
\end{itemize}

Hence, at most two vertices of $H$ are in $R$, at most two vertices of $H$ are in $S$, and none are in $V(G) \setminus (H \cup R)$. Hence, $|H| \leq 4$, a contradiction.  
\end{proof}

